Adversarial Training in Affective Computing and Sentiment Analysis: Recent Advances and Perspectives

Over the past few years, adversarial training has become an extremely active research topic and has been successfully applied to various Artificial Intelligence (AI) domains. As a potentially crucial technique for the development of the next generation of emotional AI systems, we herein provide a comprehensive overview of the application of adversarial training to affective computing and sentiment analysis. Various representative adversarial training algorithms are explained and discussed accordingly, aimed at tackling diverse challenges associated with emotional AI systems. Further, we highlight a range of potential future research directions. We expect that this overview will help facilitate the development of adversarial training for affective computing and sentiment analysis in both the academic and industrial communities.

==> cycleGAN.tex <==
% \documentclass{article}
% 
% \PassOptionsToPackage{dvipsnames}{xcolor}
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,fit,petri,backgrounds,decorations.pathmorphing,calc,shapes,shapes.misc, arrows, decorations.markings}
% 
% \usepackage[active,tightpage]{preview}
% \setlength\PreviewBorder{2pt}
% \PreviewEnvironment{tikzpicture}
% 
% \usepackage[latin1]{inputenc}
% 
% \usepackage{amsmath}
% \usepackage{amssymb}
% \newcommand{\mb}{\mathbf}
% \newcommand{\mc}{\mathcal}
% 
% \begin{document}
% \pagestyle{empty}

   \def\hsep{2cm}
   \def\vsep{1.2cm}
   \begin{tikzpicture}[shorten >=0pt,->,>=stealth, draw=black!60, node distance=\hsep, line width=1pt]
  
      \tikzstyle{object} = [rectangle, draw, fill=white, minimum height=3em, minimum width=5em, inner sep=0pt, align=center];
      \tikzstyle{action} = [circle, draw, text width=0.3cm,font=\small, inner sep=0pt,text centered];
      \tikzstyle{annot} = [rectangle, draw, text width=0.9cm, minimum height=0.8cm, text centered, inner xsep=0pt];
      \tikzstyle{net} = [trapezium, fill=gray!20!white, trapezium angle=75, draw, inner xsep=0pt, outer sep=0pt, minimum height=8mm, text width=6mm,text centered];
      \tikzstyle{dot} = [draw,circle, scale=1];
      \tikzstyle{symbol} = [text centered, text width=1.4cm]; 
      
      
      
      \node[net, rotate=-90] (Gab) {G$_{AB}$}; 
      \node[annot, above left=0.0cm and 2cm of Gab] (Sa) {$\bs{S}_A$}; 
      \node[annot, below of=Sa, node distance=\vsep] (Sbab) {$\bs{S}_{BAB}$}; 
      \node[annot, right of=Gab] (Sab) {$\bs{S}_{AB}$};
      \node[net, right of=Sab, rotate=90] (Db) {\rotatebox[origin=c]{180}{D$_B$}};
      
      \node[net, below of=Gab, rotate=-90] (Gba) {G$_{BA}$}; 
      \node[annot, above left=-0.3cm and 2cm of Gba] (Saba) {$\bs{S}_{ABA}$}; 
      \node[annot, below of=Saba, node distance=\vsep] (Sb) {$\bs{S}_{B}$};

	  \node[annot, right of=Gba] (Sba) {$\bs{S}_{BA}$}; 
      \node[net, right of=Sba, rotate=90] (Da) {\rotatebox[origin=c]{180}{D$_A$}};
      
      
      
      
%       \node[annot, text width=1em] (start) at (-0.5,0) {$\mb{z}$};
%       \node[symbol, left of=start, node distance=1*\hsep] {latent random vector};  
%       \node[net, right of=start, rotate=-90, node distance=1.2*\hsep, fill=blue!30!white] (lstm1) {\mbox{G}};
%        \node[annot, right of=lstm1, node distance=1.2*\hsep,fill=black!30!white] (pred) {$\hat{\mb{x}}$};
%        \node[annot, below of=pred, node distance=0.6*\layersep] (label) {$\mb{x}$};
%        \node[symbol, left of=label, node distance=1.2*\hsep] {real~world sample}; 
%       \node[net, rotate=90, fill=red!30!white] (lstm2) at (3.5,-0.8) {\rotatebox[origin=c]{180}{D}};
%       \node[annot, right of=lstm2, node distance=1.5*\hsep,text width=0.4cm, minimum height=1.2cm] (end) {};
%       \node[dot, above of=end, node distance=0.25*\hsep, fill=red!50!green] (real) {}; 
%      \node[dot, below of=end, node distance=0.25*\hsep, fill=blue!50!green] (fake) {};
%      \node[right of=real, node distance=0.7*\hsep](real_text){real};
%      \node[right of=fake, node distance=0.7*\hsep](fake_text){fake};

%       \path (start) edge (lstm1) 
%       (lstm1) edge (pred)
%       (lstm2) edge (end); 
%       \draw [->] (pred.east)  to ($(pred.east)+(0.4cm,0cm)$) to ($(pred.east)+(0.4cm,-0.5cm)$) to ($(lstm2.north)+(0cm,0.3cm)$);
%        \draw [->] (label.east)  to ($(label.east)+(0.4cm,0cm)$) to ($(label.east)+(0.4cm,0.7cm)$) to ($(lstm2.north)+(0cm,-0.3cm)$);

      
   \end{tikzpicture}

% \end{document}

==> ganAlgorithm.tex <==
\begin{algorithm}[!t]
\begin{algorithmic}[1]
\sFor{number of training iterations}{
	\sFor{$k$ steps}{
		\begin{itemize}
		\item Sample minibatch of $m$ noise samples ${\bs{z}^{(1)}, \ldots, \bs{z}^{(m)}}$ from noise prior $p_g(\bs{z})$.
        \item Sample minibatch of $m$ examples  ${\bs{x}^{(1)}, \ldots, \bs{x}^{(m)}}$ from data generating distribution $p_{data}(\bs{x})$.
        \item Update the discriminator by ascending its stochastic gradient:
        \begin{equation*}
        \nabla_{\theta_d}\frac{1}{m}\sum_{i=1}^{m}[logD(\bs{x}^i)+log(1-D(G(\bs{z}^{(i)})))].
        \end{equation*}
		\end{itemize}
    }
    
    \begin{itemize}
    \item Sample minibatch of $m$ noise samples ${\bs{z}^{(1)}, \ldots, \bs{z}^{(m)}}$ from noise prior $p_g(\bs{z})$.
    \item Update the generator by descending its stochastic gradient: 
    \end{itemize}
    \begin{equation*}
    \nabla_{\theta_g}\frac{1}{m}\sum_{i=1}^{m}log(1-D(G(\bs{z}^{(i)}))).
    \end{equation*}
}

The gradient-based updates can use any standard gradient-based learning rule. 
\end{algorithmic}
\caption{Training algorithm of Generative Adversarial Networks (GAN) using stochastic gradient descent. $k$: the number of steps to apply to the discriminator.~\cite{Goodfellow14-GAN}}
\label{fig:ganTraining}
\end{algorithm}

